Hierarchical Relation-augmented Representation Generalization for Few-shot Action Recognition

Few-shot action recognition (FSAR) aims to recognize novel action categories with few exemplars. Existing methods typically learn frame-level representations for each video by designing inter-frame temporal modeling strategies or inter-video interaction at the coarse video-level granularity. However, they treat each episode task in isolation and neglect fine-grained temporal relation modeling between videos, thus failing to capture shared fine-grained temporal patterns across videos and reuse temporal knowledge from historical tasks. In light of this, we propose HR2G-shot, a Hierarchical Relation-augmented Representation Generalization framework for FSAR, which unifies three types of relation modeling (inter-frame, inter-video, and inter-task) to learn task-specific temporal patterns from a holistic view. Going beyond conducting inter-frame temporal interactions, we further devise two components to respectively explore inter-video and inter-task relationships: i) Inter-video Semantic Correlation (ISC) performs cross-video frame-level interactions in a fine-grained manner, thereby capturing task-specific query features and enhancing both intra-class consistency and inter-class separability; ii) Inter-task Knowledge Transfer (IKT) retrieves and aggregates relevant temporal knowledge from the bank, which stores diverse temporal patterns from historical episode tasks. Extensive experiments on five benchmarks show that HR2G-shot outperforms current top-leading FSAR methods.

==> tabs/ab_study.tex <==


\begin{table*}
\caption{A set of ablation studies on SSv2-small~\cite{goyal2017something} and HMDB51~\cite{kuehne2011hmdb} under the $5$-way $1$-shot setting~(\S\ref{ex::abs}). The adopted network designs are marked in \textcolor{red}{red}.}
        \centering
	%\hspace{-0.7em}
	       \begin{subtable}{0.49\linewidth}
         \centering
           %\vspace{-0.4cm}
		\resizebox{\textwidth}{!}{
\setlength\tabcolsep{9.0pt}
\renewcommand\arraystretch{1.1}
\begin{tabular}{c|cc}
\thickhline
\rowcolor{mygray}
 Method  & SSv2-small & HMDB51  \\ \hline  \hline
  support-support        & $58.7$ & $84.7$     \\  
       query-support        & $59.0$ & $84.5$    \\ 
       full        & $57.8$ & $84.0$    \\
 \textcolor{red}{Ours}          & $\mathbf{60.2}$ & $\mathbf{85.6}$     \\ \hline
\end{tabular}} %\vspace{-0.3cm}
\caption{Masked Interaction Strategy}
\label{tab::mask}
	\end{subtable} 
        \hspace{0.3em}     
\begin{subtable}{0.49\linewidth}
  %\vspace{+1px}
  \centering
        \small
		\resizebox{\textwidth}{!}{
\setlength\tabcolsep{9.3pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{c|cc}
\thickhline
\rowcolor{mygray}
 Retrieval ratio $\kappa$ & SSv2-small & HMDB51  \\ \hline  \hline
  $\kappa=0.3$         & $58.9$   & $84.3$   \\  
       $\kappa=0.5$        & $59.5$   & $84.9$  \\ 
   \textcolor{red}{$\kappa=0.7$}      & $\mathbf{60.2}$   & $\mathbf{85.6}$     \\ 
$\kappa=0.9$      & $59.9$    & $85.3$     \\ 
 $\kappa=1.0$      & $59.7$    & $85.2$     \\       \hline
\end{tabular}} %\vspace{-0.3cm}
\caption{Retrieval Ratio}
\label{tab::retrival}
	\end{subtable} \\
 	\begin{subtable}{0.49\linewidth}
  \vspace{+1px}
  \centering
        \small
		\resizebox{\textwidth}{!}{
\setlength\tabcolsep{7pt}
\renewcommand\arraystretch{1.07}
\begin{tabular}{c|cc}
\thickhline
\rowcolor{mygray}
 Prototype Number $M$ & SSv2-small  & HMDB51 \\ \hline  \hline
  $M=1$         & $59.0$    & $84.7$    \\  
       $M=2$        & $59.5$   & $85.0$    \\ 
   \textcolor{red}{$M=3$}      & $\mathbf{60.2}$   & $\mathbf{85.6}$       \\ 
$M=4$      & $59.6$     & $85.3$      \\ 
 $M=8$      & $58.8$      & $85.2$     \\       \hline
\end{tabular}} %\vspace{-0.3cm}
\caption{Prototype Number}
\label{tab::pro_num}
	\end{subtable}
        \hspace{-0.7em}
	\begin{subtable}{0.49\linewidth}
 \vspace{+1px}
  \centering
        \small
		\resizebox{\textwidth}{!}{
\setlength\tabcolsep{3.7pt}
\renewcommand\arraystretch{1.02}
\begin{tabular}{c|cc}
\thickhline
\rowcolor{mygray}
 Momentum Coefficient $\mu$ & SSv2-small & HMDB51  \\ \hline  \hline
  $\mu=0$         & $57.2$    & $83.1$     \\  
       $\mu=0.5$       & $59.0$   & $84.4$     \\ 
   $\mu=0.9$      & $59.4$       & $85.0$     \\ 
\textcolor{red}{$\mu=0.99$}      & $\mathbf{60.2}$    & $\mathbf{85.6}$       \\ 
 $\mu=0.999$      & $59.9$        & $85.4$    \\       \hline
\end{tabular}} %\vspace{-0.3cm}
\caption{Momentum Coefficient}
\label{tab::mome}
	\end{subtable}
\vspace{-0.4cm}
\end{table*}


==> tabs/bank_size.tex <==
\begin{table}
%\vspace{-0.4cm}
\vspace{-0.1cm}
\centering
\small
\resizebox{0.3\textwidth}{!}{
\setlength\tabcolsep{6pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{c|c}
\thickhline
\rowcolor{mygray}
 Bank size $G$ & SSv2-small   \\ \hline  \hline
  $10$         & $59.0$      \\  
       $30$        & $59.7$     \\ 
   $50$      & $60.2$         \\ 
$80$      & $60.0$         \\ 
 $100$      & $59.9$         \\       \hline
\end{tabular}} %\vspace{-0.3cm}
\caption{Bank Size}
\label{tab::banksize}\vspace{-8pt}
\end{table}

==> tabs/interaction.tex <==
\begin{table}
%\vspace{-0.4cm}
\vspace{-0.1cm}
\centering
\small
\resizebox{0.3\textwidth}{!}{
\setlength\tabcolsep{6pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{c|cc}
\thickhline
\rowcolor{mygray}
 Method  & SSv2-small & HMDB51  \\ \hline  \hline
  within-support        & $58.7$ & $84.7$     \\  
       query-support        & $59.0$ & $84.5$    \\ 
       full        & $xx$ & $xxx$    \\
 Ours          & $\mathbf{60.2}$ & $\mathbf{85.6}$     \\ \hline
\end{tabular}} %\vspace{-0.3cm}\vspace{-12pt}
\caption{Masked Interaction Strategy}
\label{tab::mask}
\end{table}

==> tabs/pro_num.tex <==
\begin{table*}[t]
%\vspace{-0.4cm}
\vspace{-0.1cm}
\centering
\small
\resizebox{0.3\textwidth}{!}{
\setlength\tabcolsep{6pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{c|c}
\thickhline
\rowcolor{mygray}
 Prototype Number $M$ & SSv2-small   \\ \hline  \hline
  $K=1$         & $xxx$      \\  
       $K=2$        & $xxx$     \\ 
   $K=3$      & $xxx$         \\ 
$K=4$      & $xxx$         \\ 
 $K=8$      & $xxx$         \\       \hline
\end{tabular}} %\vspace{-0.3cm}
\caption{Prototype Number}\vspace{-12pt}
\label{tab::pro_num}
\end{table}

==> tabs/retrival.tex <==
\begin{table*}[t]
%\vspace{-0.4cm}
\caption{}
\vspace{-0.1cm}
\centering
\small
\resizebox{0.3\textwidth}{!}{
\setlength\tabcolsep{6pt}
\renewcommand\arraystretch{0.95}
\begin{tabular}{c|c}
\thickhline
\rowcolor{mygray}
 Retrieval ratio $\kappa$ & SSv2-small   \\ \hline  \hline
  $0.3$         & $58.9$      \\  
       $0.5$        & $59.5$     \\ 
   $0.7$      & $60.2$         \\ 
$0.9$      & $59.9$         \\ 
 $1.0$      & $59.7$         \\       \hline
\end{tabular}} \vspace{-12pt}
\caption{Retrieval Ratio}
\label{tab::retrival}`
\end{table*}

==> tabs/sota.tex <==
\begin{table*}[t]
\caption{Quantitative results on SSv2-small~\cite{goyal2017something}, SSv2-full~\cite{goyal2017something}, HMDB51~\cite{kuehne2011hmdb}, UCF101~\cite{soomro2012ucf101}, and Kinetics~\cite{carreira2017quo} (see \S\ref{sec::sota}). ``INet-RN50” denotes ResNet-50 pre-trained on ImageNet. The best results are highlighted.}
\label{tab::sota}
\small
\resizebox{1.0\linewidth}{!}{
\setlength\tabcolsep{5.5pt}
\renewcommand\arraystretch{1.05}
\begin{tabular}{l|c||c|cc|cc|cc|cc|cc}
\thickhline
\rowcolor{mygray}    &  & & \multicolumn{2}{c|}{SSv2-small}& \multicolumn{2}{c|}{SSv2-full} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c}{Kinetics} \\ 
\rowcolor{mygray}          \multirow{-2}*{Method}   & \multirow{-2}*{Reference}   & \multirow{-2}*{Pre-training}         &$1$-shot         & $5$-shot   & $1$-shot       & $5$-shot   & $1$-shot      & $5$-shot &$1$-shot         & $5$-shot &$1$-shot         & $5$-shot \\ \hline\hline
CMN~\cite{zhu2018compound}  & ECCV'18    &  INet-RN50   &$34.4$& $43.8$& $36.2$ &$48.9$      & -       & -      & -       & -      & $60.5$ &$78.9$      \\
OTAM~\cite{cao2020few}   & CVPR'20   &  INet-RN50 & -& -& $42.8$ &$52.3$& - &-& -& - &$73.0$& $85.8$
    \\
AmeFuNet~\cite{fu2020depth} & MM’20 &INet-RN50&  - &- &-& -& $60.2$ &$75.5$& $85.1$ &$95.5$& $74.1$ &$86.8$  \\
TRX~\cite{perrett2021temporal}  & CVPR'21    &  INet-RN50   & - &$59.1$ &- &$64.6$& - &$75.6$ &- &$96.1$& $63.6$ &$85.9$\\

TA$^{2}$N~\cite{ta2n}   & AAAI'22   &  INet-RN50   & -     & -       & $47.6$& $61.0$    &$59.7$& $73.9$& $81.9$& $95.1$ & $72.8$ &$85.8$   \\

MTFAN~\cite{wu2022motion}   & CVPR'22   &  INet-RN50  & -     & - & $45.7$ &$60.4$& $59.0$ & $74.6$& $84.8$ & $95.1$& $74.6$          & $87.4$     \\

HyRSM~\cite{wang2022hybrid} & CVPR'22   &  INet-RN50  & $40.6$ &$56.1$& $54.3$& $69.0$& $60.3$& $76.0$&$83.9$& $94.7$& $73.7$ &$86.1$     \\

STRM~\cite{thatipelli2022spatio}   & CVPR'22   &  INet-RN50   & $37.1$& $55.3$ &$43.1$& $68.1$&  $52.3$&  $77.3$& $80.5$ & $96.9$ &$62.9$& $86.7$ \\

HCL~\cite{zheng2022few}   & ECCV'22     &  INet-RN50 &  $38.9$& $55.4$& $47.3$ &$64.9$ &$59.1$ & $76.3$& $82.6$ & $94.5$  &$73.7$ &$85.8$ \\
MoLo~\cite{wang2023molo}   & CVPR'23    & INet-RN50    & $41.9$& $56.2$ &$55.0$& $69.6$& $60.8$& $77.4$& $86.0$& $95.5$& $74.0$ &$85.6$
  \\ 
GgHM~\cite{boosting}    & ICCV'23   & INet-RN50   & -& -&$54.5$ &$69.2$&  $85.2$ &$96.3$& $61.2$ &$76.9$&  $74.9$& $87.4$   \\ 
CLIP-FSAR~\cite{wang2024clip}  & IJCV'24    &  CLIP-RN50    & $52.0$ &$55.8$& $58.1$ &$62.8$& $69.2$&  $80.3$ &$91.3$&  $97.0$ &$87.6$& $91.9$ \\
CLIP-Freeze~\cite{radford2021learning} & ICML'21    &  CLIP-ViT-B & $29.5$& $42.5$ &$30.0$ &$42.4$ &$58.2$ & $77.0$& $89.7$ &$ 95.7$ &$78.9$ &$91.9$ \\
CapFSAR~\cite{wang2023few} & Arxiv'23    &  CLIP-ViT-B & $45.9$ &$59.9$& $51.9$& $68.2$ & $65.2$&  $78.6$ &$93.3$ & $97.8$ & $84.9$& $93.1$ \\
MVP-shot~\cite{qu2024mvp}  & Arxiv'24    &  CLIP-ViT-B  & $55.4$ & $62.0$ &- &- & $77.0$& $88.1$ &$96.8$& $99.0$& $91.0$& $95.1$ \\
MA-FSAR~\cite{xing2023multimodal}  & Arxiv'24    &  CLIP-ViT-B    &  $59.1$& $64.5$& $63.3$ &$72.3$ & $83.4$& $87.9$ &$97.2$ &$99.2$ &$\mathbf{95.7}$ &$96.0$  \\
CLIP-FSAR~\cite{wang2024clip}   & IJCV'24   &  CLIP-ViT-B    & $54.6$ &$61.8$& $62.1$ &$72.1$& $77.1$& $87.7$& $97.0$& $99.1$ &$94.8$& $95.4$  \\ 
\hline\hline
%\textbf{xxx (ours)}         & - & CLIP-RN50       & $\mathbf{xx}$    & $\mathbf{xxx}$   & $\mathbf{xxx}$   & $\mathbf{xxx}$    & $\mathbf{xx}$ & $\mathbf{xxx}$ & $\mathbf{xx}$   & $\mathbf{xx}$    & $\mathbf{xx}$   & $\mathbf{xx}$\\
 \textbf{HR$^{2}$G-shot (ours)}         & - & CLIP-ViT-B       & $\mathbf{60.2}$    & $\mathbf{66.0}$   & $\mathbf{65.4}$   & $\mathbf{74.8}$    & $\mathbf{85.6}$ & $\mathbf{88.6}$ & $\mathbf{98.0}$   & $\mathbf{99.3}$    & 95.2   & $\mathbf{96.4}$ \\ \hline
\end{tabular}}\vspace{-12pt}
\end{table*}
